Simultaneous determination of the cosmic birefringence and miscalibrated polarisation angles from CMB experiments

We show that the cosmic birefringence and miscalibrated polarisation angles can be determined simultaneously by cosmic microwave background (CMB) experiments using the cross-correlation between $E$- and $B$-mode polarisation data. This is possible because polarisation angles of the CMB are rotated by both the cosmic birefringence and miscalibration effects,whereas those of the Galactic foreground emission only by the latter. Our method does not require prior knowledge of the $E$- and $B$-mode power spectra of the foreground emission, but uses only the knowledge of the CMB polarisation spectra. Specifically, we relate the observed $EB$ correlation to the difference between the $\mathit{observed}$ $E$- and $B$-mode spectra in the sky, and use different multipole dependence of the CMB (given by theory) and foreground spectra (with no assumption) to derive the likelihood for the miscalibration angle $\alpha$ and the birefringence angle $\beta$. We show that a future satellite mission similar to LiteBIRD can determine $\beta$ with a precision of ten arcminutes.

==> GeneralFitting.tex <==
If the rotation angle is large, residual terms cannot be neglected.
As an example, let us think about a term, $-E^\mathrm{CMB}E^\mathrm{N}\sin(2\alpha-2\beta)$, in Eq.~(\ref{eq:EBObsWithResiduals}).
If we neglect this term, that forces $-E^\mathrm{CMB}E^\mathrm{N}\sin(2\alpha-2\beta)$ to be zero.
However, in a statistical fluctuation, $E^\mathrm{CMB}E^\mathrm{N}$ takes non-zero value.
In such case, this term give a bias, $\sin(2\alpha-2\beta)=0$.
To mitigate this bias, it is needed to fit all the residual terms.
Including CMB term, the full likelihood is prepared as 
\begin{equation}\label{eq:LikelihoodGeneral}
\begin{split}
\mathcal{L} &= \prod_{\ell=2}^{\ell_\mathrm{max}}\exp\left[
\frac{
	\left(
	\splitdfrac{
		C_\ell^{EB,\mathrm{o}} 
		- \frac{\tan(4\alpha)}{2} \left(C^{EE,\mathrm{obs}}-C^{BB,\mathrm{obs}}\right) 	
	}{
		-  \frac{\sin(4\alpha+4\beta)}{2\cos(4\alpha + 4\gamma)}
		\left(
		C_{\ell}^{EE,\mathrm{CMB,int}} - C_{\ell}^{BB,\mathrm{CMB,int}} 
		\right)	
		-\sum_{s=3}^\mathrm{residuals} a_s x_s
	}
	\right)^2
}{
	\Var( C_\ell^{ EB, \mathrm{o} } ) 
	+ 
	\Var\left(C^{EE,\mathrm{obs}}-C^{BB,\mathrm{obs}}\right) \frac{\tan^2(4\alpha)}{2^2}
}
\right]\\
&\cdot 
\exp\left[
\frac{ 
	\left(C_{\ell}^{EE,\mathrm{CMB,int}} - C_\ell^{EE,\mathrm{CMB,th} } \right)^2 
}{2\Var( C_\ell^{EE,\mathrm{CMB,th} } ) 
}
\right]
\cdot
\exp\left[
\frac{ 
	\left(C_\ell^{BB,\mathrm{CMB,int}} - C_\ell^{BB,\mathrm{CMB,th} } \right)^2 
}{2\Var( C_\ell^{BB,\mathrm{CMB,th} } ) 
}
\right]\\
\cdot & 
\prod_{s=3}^{\mathrm{residuals}}
\exp\left[
\frac{ \left(x_s - \bar{x_s}(=0)\right)^2}{2\Var(x_s)}
\right]
,
\end{split}
\end{equation}
where $x_s$ and $a_s$ are a residual term and its coefficient.
If we express $C_\ell^{EE,\mathrm{CMB,int}}$  and  $C_\ell^{BB,\mathrm{CMB,int}}$ as $x_1$ and $x_2$ for each, general log-likelihood is expressed as
\begin{equation}\label{eq:LogLikelihoodGeneral}
\begin{split}
-\ln \mathcal{L}&= \sum_{\ell=2}^{\ell_\mathrm{max}}\left[\frac{ \left(z - y -\sum_{s=1}^{n} a_s x_s \right)^2}{ 2 (\Var(z) + \Var(y) )}
+ \sum_{s=1}^{n} \frac{ \left(x_s - \bar{x_s}\right)^2}{2\Var(x_s)}\right],
\end{split}
\end{equation}
where $z = C_\ell^{EB,\mathrm{o}}$, and $y=\frac{\tan(4\alpha)}{2} 
\left(C_\ell^{EE,\mathrm{obs}}-C_\ell^{BB,\mathrm{obs}}\right) $, and $n=19$.
For the estimation of angles, this log-likelihood need to be minimized.


\begin{comment}
From Eq~\ref{eq:EBandEEBB_obs}, we can measure miscalibration angle, $\alpha$, without the assumption of intrinsic $C_\ell^{EE} - C_\ell^{BB}$.
However, we know the intrinsic $C_\ell^{EE, \mathrm{CMB}} - C_\ell^{BB, \mathrm{CMB}}$ without intordial $B-$mode.
These mean that we can estimate one additional angle rotation to CMB or foregrounds.
In this paper, birefringence rotation is \TODO denoted as $\beta$ and rotation angle of foregrounds are \TODO denoted as $\gamma$.
The general expression of fitting with all angles are shown as Eq.~\ref{eq:GeneralRotationFitting}.
We can estimate birefringence angle $\beta$, if we assume no rotation in foregrounds.
And we can estimate foreground rotation-angle $\gamma$, if we assume no rotation in CMB.
\TODO Here we would like to note that we only know the centre value of CMB power spectra, even though we only can observe one realization.
Therefore we need to consider the cosmic variance to fit CMB terms. 
The log likelihood is as 
%Eq.~\ref{eq:EBandEEBB_obs}
\begin{equation}\label{eq:GeneralLogLikelihood}
\begin{split}
-\ln \mathcal{L}&= \sum_{\ell=2}^{ \ell_\mathrm{max} }\frac{
	 \left(C_\ell^{EB, \mathrm{o}} - 
	\frac{\tan(4\alpha + 4\gamma) }{2}
	\left(C_{\ell}^{EE,\mathrm{o}}-C_{\ell}^{BB,\mathrm{o}}\right)
%	 -\sum_{s=1}^{n} a_s x_s 
	- 
	\frac{\sin(4\alpha+4\beta)}{2\cos(4\alpha + 4\gamma)}
	\left(C_{\ell}^{EE,\mathrm{CMB,int}} - C_{\ell}^{BB,\mathrm{CMB,int}} \right)
	\right)^2
	}{2\Var(C_\ell^{EB, \mathrm{o}})}
\\&
+ \frac{ 
 	\left(C_{\ell}^{EE,\mathrm{CMB,int}} - C_\ell^{EE,\mathrm{CMB,theory} } \right)^2 
 }{2\Var( C_\ell^{EE,\mathrm{CMB,theory} } ) 
}
+ \frac{ 
	\left(C_\ell^{BB,\mathrm{CMB,int}} - C_\ell^{BB,\mathrm{CMB,theory} } \right)^2 
}{2\Var( C_\ell^{BB,\mathrm{CMB,theory} } ) 
},
\end{split}
\end{equation}
where ``int'' means intrinsic CMB of one realization.
And here, we calculated $\Var(C_\ell^{XX, CMB, theory})$($XX=EE,\ BB$) as $2 {C_\ell^{XX, CMB, theory} }^2/(2\ell+1)$.
\subsection{Measurement of birefringence angle}
If we assume foreground rotation $\gamma$ to be zero and would like to estimate $\beta$, we only need to set $\gamma=0$ in Eq.~\ref{eq:GeneralRotationFitting}.
\subsection{Measurement of angle rotation in foregrounds}
If we assume birefringence rotation $\beta$ to be zero and would like to estimate foreground rotation $\gamma$, we only need to set $\beta=0$ in Eq.~\ref{eq:GeneralRotationFitting}.
\end{comment}


==> Residuals.tex <==
In this section, we will show all the terms of $C_\ell^{EB, \mathrm{obs}}$.
$E$- and $B$-modes with angle rotations by miscalibration ($\alpha$), birefringence ($\beta$), and foregrounds $EB$ correlation ($\gamma$) are presented as
\begin{align}
E^\mathrm{obs} &= 
E^\mathrm{fg}\cos(2\alpha+2\gamma)-  B^\mathrm{fg}\sin(2\alpha+2\gamma)
+E^\mathrm{CMB}\cos(2\alpha+2\beta)-  B^\mathrm{CMB}\sin(2\alpha+2\beta)
+E^\mathrm{N},
\\
B^\mathrm{obs} &= 
E^\mathrm{fg}\sin(2\alpha + 2\gamma) + B^\mathrm{fg}\cos(2\alpha + 2\gamma)
+E^\mathrm{CMB}\sin(2\alpha+2\beta) + B^\mathrm{CMB}\cos(2\alpha+2\beta)
+B^\mathrm{N},	 
\end{align}
where ``obs" means observed, fg means foregrounds, and N means noise.
Using these expressions, we can calculate relational expression of correlations as
\begin{equation}
\begin{split}
\left( C^{EB,\mathrm{obs}}\right.&
\left.
-\frac{\tan(4\alpha + 4\gamma) }{2}
\left(C^{EE,\mathrm{obs}}-C^{BB,\mathrm{obs}}\right)
\right)\cos(4\alpha + 4\gamma) =
\\&
(C^{EE,\mathrm{CMB}} - C^{BB,\mathrm{CMB}})\sin(4\beta)/2\\&
+C^{EB, \mathrm{fg}}+ C^{EB, \mathrm{N}} \cos(4\alpha + 4\gamma) + C^{EB,\mathrm{CMB}}\cos(4\beta)\\&
-(C^{EE, \mathrm{N}} - C^{BB, \mathrm{N}})\sin(4\alpha +4\gamma)/2\\&
+(E^\mathrm{fg}B^\mathrm{CMB} + B^\mathrm{fg}E^\mathrm{CMB}) \cos( 2\beta)
+ (E^\mathrm{fg}E^\mathrm{CMB} - B^\mathrm{fg}B^\mathrm{CMB})\sin(2\beta)\\&
+ (E^\mathrm{fg}B^\mathrm{N} + B^\mathrm{fg} E^\mathrm{N}) \cos(2\alpha + 2\gamma)
-(E^\mathrm{fg}E^\mathrm{N}- B^\mathrm{fg}B^\mathrm{N} )\sin(2\alpha)\\&
+(E^\mathrm{CMB}B^\mathrm{N}+ B^\mathrm{CMB}E^\mathrm{N} )\cos(2\alpha +2\gamma -2\beta)\\&
-(E^\mathrm{CMB}E^\mathrm{N} - B^\mathrm{CMB}B^\mathrm{N})\sin(2\alpha +2\gamma -2\beta)\\&
\end{split}
\end{equation}
Here, non-stochastic terms, which take non-zero value in ensemble average, are
\begin{comment}
\begin{equation}
\begin{split}C^{EB,\mathrm{o}} &=
\left(
C^{EE,\mathrm{fg}} - C^{BB,\mathrm{fg}} 
\right)
\frac{1}{2}\sin(4\alpha)
+
C^{EB, \mathrm{fg}}\cos(4\alpha+4\gamma)
\\&
+
\left(
C^{EE,\mathrm{CMB}} - C^{BB,\mathrm{CMB}} 
\right)
\frac{1}{2}\sin(4\alpha+4\beta)
+
C^{EB,\mathrm{CMB}}\cos(4\alpha+4\beta)
\\
&+
\left(
E^\mathrm{fg}E^{\mathrm{CMB}}
-
B^\mathrm{fg}B^{\mathrm{CMB}}
\right)\sin(4\alpha+2\beta)
\\
&
+\left(
E^\mathrm{fg}B^{\mathrm{CMB}}
+B^\mathrm{fg}E^{\mathrm{CMB}}
\right)\cos(4\alpha+2\beta+2\gamma)
\\
&
+(E^\mathrm{fg}E^\mathrm{N}-  B^\mathrm{fg}E^\mathrm{N})\sin(2\alpha+2\gamma)
\\
&
+(E^\mathrm{fg}B^\mathrm{N}+ B^\mathrm{fg}E^\mathrm{N})\cos(2\alpha + 2\gamma)\\
&
+(E^\mathrm{CMB}E^\mathrm{N}-  B^\mathrm{CMB}E^\mathrm{N})\sin(2\alpha+2\beta)
\\
&
+(E^\mathrm{CMB}B^\mathrm{N}+ B^\mathrm{CMB}E^\mathrm{N})\cos(2\alpha+2\beta)\\
&
+E^\mathrm{N}B^\mathrm{N}.
\end{split}
\end{equation}
\end{comment}

\begin{equation}\label{eq:GeneralRotationFitting}
\begin{split}
C^{EB,\mathrm{o}} &=
\frac{\tan(4\alpha + 4\gamma) }{2}
\left(C^{EE,\mathrm{o}}-C^{BB,\mathrm{o}}\right)
+
\frac{\sin(4\alpha+4\beta)}{2\cos(4\alpha + 4\gamma)}\left(
C^{EE,\mathrm{CMB}} - C^{BB,\mathrm{CMB}} 
\right) .
\end{split}
\end{equation} 
Therefore, we fit $C_\ell^{EB, \mathrm{o}}$ with $C_\ell^{EE,\mathrm{o}}- C_\ell^{BB, \mathrm{o}}$ and $C_\ell^{EE,\mathrm{CMB}}- C_\ell^{BB, \mathrm{CMB}}$ to estimate angles.
Since we have only two components to fit $C_\ell^{EB, \mathrm{o}}$, we can estimate combinations of ($\alpha$, $\beta$) or ($\alpha$, $\gamma$).


==> Variance_old.tex <==
In this section, we describe the treatment of variance  of $C_\ell^{EB, \mathrm{o}}   - ( C_\ell^{EE, \mathrm{o}} - C_\ell^{BB, \mathrm{o}})\tan(4\alpha)/2 $ in Eq.~(\ref{eq:LikelihoodGeneral}).
For simplicity, only for this section, we write spherical harmonics coefficients of the observed $E$- and $B$-mode polarisation as 
\begin{align}
E_{\ell,m}^\mathrm{obs}&= \sum_{i} E_{\ell,m,i},
\\
B_{\ell,m}^\mathrm{obs}&= \sum_{i} B_{\ell,m,i},
\end{align}
where $i$ denotes each component: CMB, foregrounds, and noise.
Here, these coefficients are the rotated ones.

Ensemble average of $C_\ell^{EB, \mathrm{o}}   - ( C_\ell^{EE, \mathrm{o}} - C_\ell^{BB, \mathrm{o}})\tan(4\alpha)/2 $
is calculated as
\begin{equation}\label{square}
\begin{split}
\langle C_\ell^{EB, \mathrm{o}} -& ( C_\ell^{EE, \mathrm{o}} - C_\ell^{BB, \mathrm{o}})\tan(4\alpha)/2  \rangle \\
&=  \sum_{i,j}\left[
\langle C_\ell^{E_i B_j , \mathrm{o}} \rangle \delta_{i,j}   - ( \langle C_\ell^{E_i E_j, \mathrm{o}} \rangle \delta_{i,j} - \langle  C_\ell^{B_i B_j , \mathrm{o}} \rangle \delta_{i,j} )\tan(4\alpha)/2 
\right]
\\
&=
\sum_{i}\left[
\langle C_\ell^{EB_i, \mathrm{o}} \rangle   - ( \langle C_\ell^{EE_i, \mathrm{o}} \rangle - \langle  C_\ell^{BB_i, \mathrm{o}} \rangle )\tan(4\alpha)/2 
\right],
\end{split}
\end{equation}
where we assume cross-correlation between different terms vanish in ensemble average.

Therefore square of ensemble average becomes
\begin{equation}\label{eq:SquareAverage}
\begin{split}
\langle C_\ell^{EB, \mathrm{o}} -& ( C_\ell^{EE, \mathrm{o}} - C_\ell^{BB, \mathrm{o}})\tan(4\alpha)/2  \rangle^2
\\
&= 
\sum_{i,j} 
\left[
\langle C_\ell^{EB, i} \rangle   - ( \langle C_\ell^{EE, i} \rangle 
- \langle  C_\ell^{BB, i} \rangle )\tan(4\alpha)/2 
\right]
\\
&\cdot
\left[
\langle C_\ell^{EB,j} \rangle   - ( \langle C_\ell^{EE, j} \rangle - \langle  C_\ell^{BB, j} \rangle )\tan(4\alpha)/2 
\right]
\\
&=
\sum_{i,j}
\left[
\langle C_\ell^{EB, i} \rangle \langle C_\ell^{EB, j} \rangle
+ \frac{\tan^2(4\alpha)}{4} \langle C_\ell^{EE, i } \rangle  \langle C_\ell^{EE, j} \rangle
+ \frac{\tan^2(4\alpha)}{4} \langle  C_\ell^{BB, i} \rangle \langle  C_\ell^{BB, j} \rangle
\right.
\\
&\left.
- \tan(4\alpha) \langle  C_\ell^{EB, i} \rangle \langle  C_\ell^{EE, j} \rangle
+ \tan(4\alpha) \langle  C_\ell^{EB, i} \rangle \langle  C_\ell^{BB, j} \rangle
- \frac{\tan^2(4\alpha)}{2} \langle  C_\ell^{EE, i} \rangle \langle  C_\ell^{BB, j} 
\rangle
\right]
\end{split}
\end{equation}

Next, mean square of  $C_\ell^{EB, \mathrm{o}}   - ( C_\ell^{EE, \mathrm{o}} - C_\ell^{BB, \mathrm{o}})\tan(4\alpha)/2 $ is calculated as
\begin{equation}\label{eq:meansquare}
\begin{split}
\langle 
\left[ 
	C_\ell^{EB, \mathrm{o}}   
\right. 
	& 
\left. 
	- ( C_\ell^{EE, \mathrm{o}} - C_\ell^{BB, \mathrm{o}})\tan(4\alpha)/2 
\right]^2 \rangle =
\\&
\frac{1}{ (2\ell+1)^2 }
\sum_{i,j} \sum_{i',j'}
\langle E_{\ell,m,i} B_{\ell,m,j} E_{\ell,m,i'} B_{\ell,m,j'}\rangle
+\frac{\tan^2(4\alpha)}{4}\langle E_{\ell,m,i} E_{\ell,m,j} E_{\ell,m,i'} E_{\ell,m,j'}\rangle
\\&
+\frac{\tan^2(4\alpha)}{4}\langle B_{\ell,m,i} B_{\ell,m,j} B_{\ell,m,i'} B_{\ell,m,j'}\rangle
- \tan(4\alpha) \langle E_{\ell,m,i} B_{\ell,m,j} E_{\ell,m,i'} E_{\ell,m,j'}\rangle
\\
&
+ \tan(4\alpha) \langle E_{\ell,m,i} B_{\ell,m,j} B_{\ell,m,i'} B_{\ell,m,j'}\rangle
- \frac{\tan^2(4\alpha)}{2} \langle E_{\ell,m,i} E_{\ell,m,j} B_{\ell,m,i'} B_{\ell,m,j'}\rangle
\\&
=\sum_{i,j}
\left(
\frac{2\ell+2}{2\ell+1}  - \frac{\tan^2(4\alpha)}{2\ell+1} 
\right)
\langle  C_\ell^{EB, i} \rangle \langle  C_\ell^{EB, j} \rangle
+
\left(
\frac{1}{2\ell+1}  - \frac{\tan^2(4\alpha)}{ 2}
\right)
\langle  C_\ell^{EE, i} \rangle \langle  C_\ell^{BB, j} \rangle
\\&
+\frac{\tan^2(4\alpha)}{4}\frac{2\ell+3}{2\ell+1}\left(
\langle C_\ell^{EE, i } \rangle  \langle C_\ell^{EE, j} \rangle
+
\langle C_\ell^{BB, i } \rangle  \langle C_\ell^{BB, j} \rangle
\right) 
\\&
-\tan(4\alpha)\frac{2\ell+3}{2\ell+1} \langle  C_\ell^{EB, i} \rangle
\left(  \langle  C_\ell^{EE, j} \rangle -  \langle  C_\ell^{BB, j} \rangle
\right).
\end{split}
\end{equation}

From Eq.~(\ref{eq:SquareAverage}) and Eq.~(\ref{eq:meansquare}), 
\begin{equation}
\begin{split}
\Var (C_\ell^{EB, \mathrm{o}}   - ( C_\ell^{EE, \mathrm{o}} - C_\ell^{BB, \mathrm{o}})\tan(4\alpha)/2 ) &=
\sum_{i,j}
\frac{1}{2\ell+1}\langle  C_\ell^{EE, i} \rangle \langle  C_\ell^{BB, j} \rangle
\\&
+\frac{\tan^2(4\alpha)}{4}\frac{2}{2\ell+1}\left(
\langle C_\ell^{EE, i } \rangle  \langle C_\ell^{EE, j} \rangle
+
\langle C_\ell^{BB, i } \rangle  \langle C_\ell^{BB, j} \rangle
\right) 
\\
&
-\tan(4\alpha)\frac{2}{2\ell+1} \langle  C_\ell^{EB, i} \rangle
\left(  \langle  C_\ell^{EE, j} \rangle -  \langle  C_\ell^{BB, j} \rangle
\right)
\\
&+\frac{1}{2\ell+1}
\left(
1 - \tan^2(4\alpha) 
\right)
\langle  C_\ell^{EB, i} \rangle \langle  C_\ell^{EB, j} \rangle.
\end{split}
\end{equation}
Here $\langle  C_\ell^{EB, i} \rangle$ terms is created from a rotation of primordial $E$- and $B$-modes as
\begin{equation}
\langle  C_\ell^{EB, i} \rangle = \frac{1}{2} \left(  \langle \tilde{C}_\ell^{EE, i} \rangle - \langle \tilde{C}_\ell^{BB,i} \rangle \right) \sin(4 \psi_i ),
\end{equation}
where $\tilde{C}$ denotes primordial power spectrum and $\psi_i $ denotes the rotation angle for i-th component.
Then, $\langle  C_\ell^{EB, i} \rangle \langle  C_\ell^{EB, j} \rangle$ is proportion to $\mathcal{O}(\psi_i \psi_j )$,
and can be neglected for small angles cases.
Therefore, $\Var(C_\ell^{EB, \mathrm{o}}   - ( C_\ell^{EE, \mathrm{o}} - C_\ell^{BB, \mathrm{o}})\tan(4\alpha)/2 )$ is approximated to 

\begin{equation}\label{eq:VarEBmEEmBB}
\begin{split}
\Var(C_\ell^{EB, \mathrm{o}}   - ( C_\ell^{EE, \mathrm{o}} - C_\ell^{BB, \mathrm{o}})\tan(4\alpha)/2 )
&=\sum_{i,j}
\frac{1}{2\ell+1}\langle  C_\ell^{EE, i} \rangle \langle  C_\ell^{BB, j} \rangle
\\&
+\frac{\tan^2(4\alpha)}{4}\frac{2}{2\ell+1}\left(
\langle C_\ell^{EE, i } \rangle  \langle C_\ell^{EE, j} \rangle
+
\langle C_\ell^{BB, i } \rangle  \langle C_\ell^{BB, j} \rangle
\right) 
\\
&
-\tan(4\alpha)\frac{2}{2\ell+1} \langle  C_\ell^{EB, i} \rangle
\left(  \langle  C_\ell^{EE, j} \rangle -  \langle  C_\ell^{BB, j} \rangle
\right).
\end{split}
\end{equation}

Moreover, we assume the $C_\ell^{EB,\mathrm{o}}$, $C_\ell^{EE,\mathrm{o}}$, and $C_\ell^{BB,\mathrm{o}}$ are close to $\langle C_\ell^{EB,\mathrm{o}}\rangle$, $\langle C_\ell^{EE,\mathrm{o}}\rangle$, and $ \langle C_\ell^{BB,\mathrm{o}}\rangle$ because the variances are small in high $\ell$ where the fitting constraint is strong.

\subsection{Extra point}
In this section, let us explain the interpretation of Eq.~(\ref{eq:VarEBmEEmBB}).
The Eq.~(\ref{eq:VarEBmEEmBB}) can be expressed as 
\begin{equation}\label{eq:VarbyVar}
\begin{split}
\Var(
	C_\ell^{EB, \mathrm{o}}   - ( C_\ell^{EE, \mathrm{o}} - C_\ell^{BB, \mathrm{o}})\tan(4\alpha)/2 
)
&=
\Var (C_\ell^{EB,\mathrm{o} } )
\\
&
+ \frac{\tan^2(4\alpha)}{4} 
\left(
	\Var(C_\ell^{EE,\mathrm{o} } ) + \Var( C_\ell^{BB,\mathrm{o} } )
\right) 
\\
&
-2\tan(4\alpha) \mathrm{Cov}\left(
	C_\ell^{EB, \mathrm{o} },  C_\ell^{EE, \mathrm{o}} -  C_\ell^{BB, \mathrm{o}} 
\right)
.
\end{split}
\end{equation}

